Utilizing Graph Generation for Enhanced Domain Adaptive Object Detection

The problem of Domain Adaptive in the field of Object Detection involves the transfer of object detection models from labeled source domains to unannotated target domains. Recent advancements in this field aim to address domain discrepancies by aligning pixel-pairs across domains within a non-Euclidean graphical space, thereby minimizing semantic distribution variance. Despite their remarkable achievements, these methods often use coarse semantic representations to model graphs, mainly due to ignoring non-informative elements and failing to focus on precise semantic alignment. Additionally, the generation of coarse graphs inherently introduces abnormal nodes, posing challenges and potentially biasing domain adaptation outcomes. Consequently, we propose a framework, which utilizes the Graph Generation to enhance the quality of DAOD (\method{}). Specifically, we introduce a Node Refinement module that utilizes a memory bank to reconstruct noisy sampled nodes while applying contrastive regularization to noisy features. To enhance semantic alignment, we propose separating domain-specific styles from category invariance encoded within graph covariances, which allows us to selectively remove domain-specific styles while preserving category-invariant information, thus facilitating more accurate semantic alignment across different domains. Furthermore, we propose a Graph Optimization adaptor, leveraging variational inference to mitigate the impact of abnormal nodes. Extensive experimentation across three adaptation benchmarks validates that \method{} achieves state-of-the-art performance in the task of unsupervised domain adaptation.

==> code/3_preliminary.tex <==

% \newpage
\section{Preliminaries}

\subsection{Continuous Graph Neural Networks}
Given a graph $G=(\mathcal{V},\mathcal{E})$ with the node set $\mathcal{V}$ and the edge set $\mathcal{E}$. $\mathbf{X}\in\mathbb{R}^{|\mathcal{V}|\times d}$ is the node feature matrix, $d$ is the feature dimension. The binary adjacency matrix denoted as $\mathbf{A}\in\mathbb{R}^{|\mathcal{V}|\times |\mathcal{V}|}$, where $a_{ij}=1$ denotes there exists a connection between node $i$ and $j$, and vice versa. Our goal is to learn a node representation $\mathbf{H}$ for downstairs tasks.

\textbf{First-order CGNNs}.
The first graph ODE-based CGNN method is proposed by~\cite{xhonneux2020continuous}. Considering the Simple GNN~\cite{wu2019simplifying} with $\mathbf{H}_{n+1}=\mathbf{AH}_n+\mathbf{H}_0$, the solution of the ODE is given by:
\begin{equation}
\label{first_graph_ode}
\begin{aligned}
    &\frac{d\mathbf{H}(t)}{dt}=ln\mathbf{AH}(t)+\mathbf{E},\\ \mathbf{H}(t)=(\mathbf{A}&-\mathbf{I})^{-1}(e^{(\mathbf{A}-\mathbf{I})t}-\mathbf{I})\mathbf{E}+e^{(\mathbf{A}-\mathbf{I})t}\mathbf{E},
\end{aligned}
\end{equation}
where $\mathbf{E}=\varepsilon \mathbf(X)$ is the output of the encoder $\varepsilon$ and the initial value $\mathbf{H}(0)=(ln\mathbf{A})^{-1}(\mathbf{A}-\mathbf{I})\mathbf{E}$.



\textbf{Second-order CGNNs}.
To model high-order correlations in long-term temporal trends, ~\cite{rusch2022graph} first propose the second-order graph ODE, which is represented as:
\begin{equation}
\label{second}
    \mathbf{X}^{''}=\sigma(\mathbf{F}_{\theta}(\mathbf{X},t))-\gamma \mathbf{X}-\alpha \mathbf{X}^{'},
\end{equation}
where $\left(\mathbf{F}_\theta(\mathbf{X},t)\right)_i=\mathbf{F}_\theta \left(\mathbf{X}_i(t),\mathbf{X}_j(t),t\right)$ is a learnable coupling function with parameters $\theta$. Due to the unavailability of an analytical solution for Eqn.~\ref{second}, GraphCON~\cite{rusch2022graph} addresses it through an iterative numerical solver employing a suitable time discretization method. GraphCON utilizes the IMEX (implicit-explicit) time-stepping scheme, an extension of the symplectic Euler method~\cite{book} that accommodates systems with an additional damping term. %For $n=1,\cdots,N$,
\begin{equation}
\label{second_graph_ode}
\begin{aligned}
    \mathbf{Y}^n=&\mathbf{Y}^{n-1}+\Delta t\left[\sigma(\mathbf{F}_\theta(\mathbf{X}^{n-1},t^{n-1}))\right.\\
    &\left.-\gamma\mathbf{X}^{n-1}-\alpha\mathbf{Y}^{n-1}\right],\\ \mathbf{X}^n=&\mathbf{X}^{n-1}+\Delta t\mathbf{Y}^n,\, n=1,\cdots,N,
\end{aligned}
\end{equation}
where $\Delta t>0$ is a fixed time-step and $\mathbf{Y}^n$, $\mathbf{X}^n$ denote the hidden node features at time $t^n=n\Delta t$.

\subsection{Spiking Neural Networks}
\textbf{First-order SNNs}.
% SNNs utilize binary activations in each layer, which limits the representation capacity. To address the issue, 
In contrast to traditional artificial neural networks, SNNs convert input data into binary spikes over time, with each neuron in the SNNs maintaining a membrane potential that accumulates input spikes. A spike is produced as an output when the membrane potential exceeds a threshold. And the first-order SNNs is formulated as:
% SNNs introduce a temporal dimension, known as latency $K$. In the forward pass of SNNs, inputs are presented as streams of events and repeated for $K$ time steps to produce the final result. 
% The leaky-integrate-and-fire (LIF) model is commonly used to describe the dynamics of spiking neurons. In LIF, each neuron integrates the received spikes as the membrane potential $\mathbf{u}_{\tau,i}$, which can be mathematically expressed as a first-order differential equation: 
% \begin{equation}
% \label{lif}
%     \textbf{LIF: } \bar{\lambda} \frac{d u_\tau}{d\tau} = -(u_\tau - u_{rest}) +R \cdot I(\tau), \quad u_\tau < V_{th}\ ,\nonumber
% \end{equation}
% where $u_\tau$ is the membrane potential, $I(\tau)$ is the input current, $V_{th}$ is the spiking threshold, and $R$ and $\bar{\lambda}$ are resistance and time constant, respectively. Then, we have:
% At time $\tau$, when the membrane potential $u_\tau$ reaches the spiking threshold $V_{th}$, a spike is triggered, and $u_\tau$ is reset to the resting potential $u_{\text{rest}}$, which is typically assigned a value of 0. We consider a simple current model $ I_{\tau,i} = \sum_{j} w_{ij} s_{\tau,j} + b ,$ where $w_{ij}$ is the weight from neuron $j$ to neuron $i$. Then, the general form of LIF is described as:
\begin{equation}
\begin{aligned}
    u_{\tau+1,i} = \lambda (u_{\tau,i} - &V_{th} s_{\tau,i}) + \sum_{j} w_{ij} s_{\tau,j} + b ,\\ 
% \end{equation}
% \begin{equation}
    s_{\tau+1,i} =& \mathbb{H}(u_{\tau+1,i} - V_{th}), 
\end{aligned}
\end{equation}
where $\mathbb{H}(x)$ is the Heaviside step function, which is the non-differentiable spiking function. $s_{\tau,i}$ is the binary spike train of neuron $i$, and $\lambda$ is the constant. $w_{ij}$ and $b$ are the weights and bias of each neuron. 
% The training of SNNs follows the process of BPTT, and the gradients are calculated with:
% \begin{equation}
% \label{gradient}
% \begin{aligned}
%     \frac{\partial \mathcal{L}}{\partial \mathbf{W}^l} =& \sum_{\tau=1}^K \frac{\partial \mathcal{L}}{\partial \mathbf{s}_\tau^{l+1}} \frac{\partial \mathbf{s}_\tau^{l+1}}{\partial \mathbf{u}_\tau^{l+1}}\left(\frac{\partial \mathbf{u}_\tau^{l+1}}{\partial \mathbf{W}^l}\right. \\
%     &\left.+ \sum_{k<\tau} \prod_{i=\tau-1}^k\left(\frac{\partial \mathbf{u}_{i+1}^{l+1}}{\partial \mathbf{u}_{i}^{l+1}}+\frac{\partial \mathbf{u}_{i+1}^{l+1}}{\partial \mathbf{s}_i^{l+1}}\frac{\partial \mathbf{s}_i^{l+1}}{\partial \mathbf{u}_i^{l+1}}\right)\frac{\partial \mathbf{u}_k^{l+1}}{\partial \mathbf{W}^l}\right),
% \end{aligned}
% \end{equation}
% where $\mathbf{W}^l$ is the trainable matrix on $l$-th layer and $\mathcal{L}$ is the loss. The terms $\frac{\partial \mathbf{s}_\tau^l}{\partial \mathbf{u}_\tau^l}$ are non-differentiable, and surrogate derivatives are typically used instead.

\textbf{Second-order SNNs}.
The first-order neuron models assume that an input voltage spike causes an immediate change in synaptic current, affecting the membrane potential. However, in reality, a spike leads to the gradual release of neurotransmitters from the pre-synaptic neuron to the post-synaptic neuron. To capture the temporal dynamics, we utilize the synaptic conductance-based LIF model, which considers the gradual changes in input current over time. To solve this, \cite{eshraghian2023training} propose the second-order SNN, which is formulated as:
\begin{equation}  
\label{second-order}
\left\{  
             \begin{array}{lr}  
             I_{\tau+1}=\alpha I_{\tau}+WX_{\tau+1}, &  \\  
             u_{\tau+1,i}=\beta u_{\tau,i}+I_{\tau+1,i}-R,&\\  
             s_{\tau,i}=\mathbb{H}(u_{\tau+1,i}-V_{th}), &    
             \end{array}  
\right.  
\end{equation} 
% \begin{equation}
% \label{second-order}
%     I_{\tau+1}=\alpha I_{\tau}+WX_{\tau+1},
%     u_{\tau+1,i}=\beta u_{\tau,i}+I_{\tau+1,i}-R,
%     s_{\tau,i}=\mathbb{H}(u_{\tau+1,i}-V_{th}),
% \end{equation}
where $\alpha=exp(-\Delta t/\tau_{syn})$ and $\beta=exp(-\Delta t/\tau_{mem})$, $\tau_{syn}$ models the time constant of the synaptic current in an analogous way to how $\tau_{mem}$ models the time constant of the membrane potential. 



